Automatic Abstraction in SMT-Based Unbounded Software Model Checking

Software model checkers based on under-approximations and SMT solvers are very successful at verifying safety (i.e. reachability) properties. They combine two key ideas -- (a) "concreteness": a counterexample in an under-approximation is a counterexample in the original program as well, and (b) "generalization": a proof of safety of an under-approximation, produced by an SMT solver, are generalizable to proofs of safety of the original program. In this paper, we present a combination of "automatic abstraction" with the under-approximation-driven framework. We explore two iterative approaches for obtaining and refining abstractions -- "proof based" and "counterexample based" -- and show how they can be combined into a unified algorithm. To the best of our knowledge, this is the first application of Proof-Based Abstraction, primarily used to verify hardware, to Software Verification. We have implemented a prototype of the framework using Z3, and evaluate it on many benchmarks from the Software Verification Competition. We show experimentally that our combination is quite effective on hard instances.

==> impl.tex <==
\newcommand {\wto} {<}
\newcommand {\wwto} {\le}
\newcommand {\hds}[1] {\text{{\em hds}}({#1})}
\newcommand {\ctr} {\text{{\em ctr}}}
\newcommand {\bd} {\text{{\em bound}}}
\newcommand {\nat} {\mathbb{N}}
\newcommand {\bp}[1] {\tilde{#1}}
\newcommand {\last}[1] {\text{{\em last}}({#1})}
\newcommand {\ctx}{\text{{\em ctx}}}
\newcommand {\postlem}[1]{\text{{\em post\_lemma}}({#1})}
\newcommand {\assum} {\Sigma}
\newcommand {\bvals} {\text{{\em bvals}}}
\newcommand {\core}[1] {\text{{\em core}}({#1})}
\newcommand {\ltag}[1] {N_{#1}}
\newcommand {\rtag}[2] {E_{{#1},{#2}}}
%\newcommand {\srccond}[1] {\text{{\em src-cond}}({#1})}
%\newcommand {\dstcond}[1] {\text{{\em dst-cond}}({#1})}
\newcommand {\children}[1] {\text{{\em children}}({#1})}
\newcommand {\parents}[1] {\text{{\em parents}}({#1})}

\newcounter{magicrownumbers}
\newcommand\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}}

\section {Implementation}
\label{sec:impl}



% Under-approximations
%  wto, bvars, entry, reentry, exit edges, constraints
%  maintain constraints separately from existing transition relation


% say what backedges, exit edges are

% say clearly how you want to modify the trans
% say we introduce C and B
% then say how you add extra constraints


Let $P=$\prog be the input program.  First, we transform $P$ to
$\bp{P}$ by adding new \emph{counter} variables for the loops of $P$
and adding extra constraints to the transitions to count the number of
iterations. Specifically, for each location $\ell$ we introduce a counter
variable $c_\ell$ and a bounding variable $b_\ell$. Let $C$ and $B$ be
the sets of all counter and bounding variables, respectively, and
$\bd: C \to B$ be the bijection defined as $\bd(c_\ell) = b_\ell$. We
define $\bp{P} \equiv $ \quintuple {$L$} {$\ell^o$} {$\ell^e$} {$V
  \cup C \cup B$} {$\tau \land \tau_B$}, where $\tau_B(\ell_1, \ell_2)
= \bigand X(\ell_1, \ell_2)$ and $X(\ell_1, \ell_2)$ is the smallest
set satisfying the following conditions: (a) if $\ell_1\to \ell_2$ is
a back-edge, then $\left( 0 \le c_{\ell_2}' \;\land\; c_{\ell_2}' =
c_{\ell_2}-1 \;\land\; c_{\ell_2} \le b_{\ell_2} \right) \in X(\ell_1,
\ell_2)$, (b) else, if $\ell_1 \to \ell_2$ exits the loop headed by
$\ell_k$, then $\left( c_{\ell_k}=0 \right) \in X(\ell_1, \ell_2)$ and (c)
otherwise, if $\ell_1 \to \ell_2$ is a transition inside the loop headed by
$\ell_k$, then $\left( c'_{\ell_k} = c_{\ell_k} \right) \in X(\ell_1, \ell_2)$.
%
%  {\bf AK: the rest of the
%   paragraph is wrong and needs to be fixed.} Consider an arbitrary
% transition from $\ell_1$ to $\ell_2$. If it is a back-edge, $\tau_B
% (\ell_1, \ell_2) \equiv 0 \le c_{\ell_2}' \;\land\; c_{\ell_2}' =
% c_{\ell_2}-1 \;\land\; c_{\ell_2} \le b_{\ell_2}$; If $\ell_1 \to
% \ell_2$ the exit edge for the loop at $\ell_2$, $\tau_B(\ell_1,
% \ell_2) \equiv c=0$; otherwise, $\tau_B (\ell_1, \ell_2) \equiv c'=c$.
In practice, we use optimizations to reduce the number of variables
and constraints.

This transformation preserves safety as shown below.

\begin{lemma}
\label{lem:bp_sound}
$P$ is safe iff $\bp{P}$ is safe, \ie if $\bp{\cex} = \langle \bar{\ell},
\bar{s} \rangle$ is a counterexample to $\bp{P}$, projecting $\bar{s}$
onto $V$ gives a counterexample to $P$; if $\bp{\pf}$ is a
proof of $\bp{P}$, then $\pf = \lambda \ell \cdot \{\forall B \ge 0,C \ge 0 \such
\varphi ~\mid~ \varphi \in \bp{\pf}(\ell)\}$ is a safety proof for $P$.
\end{lemma}


%\subheading{Decidable Under-approximation}
%%
%We construct $U$ from $\bp{P}$ by constraining the bound variables
%(\ie $B$) via constraints of the form $b \le \text{{\em value}}$ on
%the {\em re-entry} edges. Note that $U$ is decidable since all its
%loops are bounded.

% formal proof of decidability??

% solve box
%   used a component of mu-Z to solve decidable under-approx.
%   interface - horn clauses - so we encode U as horn clauses in the obvious way
%                               (cite Rybalchenko pldi '12)
%
%   how does the component work?
%At the heart of the
%algorithm is checking whether an expression over-approximates k-reachability for
%some value k.
%In other words, whether the expression holds for the first k steps or not.
%Moreover, this is done relative to already known expressions which hold for <=k
%steps. So, if hints
%are added as 0-step expressions, it is like having no information about them.
%Best case they will be propagated all the way to the inductive depth d.
%Otherwise, they can
%help other expressions move forward easily during the relative
%checks...something like this and not too detailed.

In the rest of this section, we define our abstractions and
under-approximations of $\bp{P}$ and describe our implementation of
the different routines in Fig.~\ref{fig:code}.

\subheading {Abstractions}
Recall that $\tau(\bp{P}) = \tau \land \tau_B$. W.l.o.g., assume that $\tau$ is
transformed to
$\exists \assum \such \left( \tau_\assum \land \bigand \assum \right)$ for a
finite set of fresh Boolean variables $\assum$ that only appear negatively in
$\tau_\assum$. We refer to $\assum$ as 
\emph{assumptions} following SAT terminology~\cite{minisat}. Dropping some
assumptions from $\bigand \assum$ results in an abstract transition relation,
\ie $\exists \assum \such \left( \tau_\assum \land
\bigand \hat{\assum} \right)$ is an abstraction of $\tau$ for $\hat{\assum}
\subseteq \assum$, denoted $\hat{\tau}(\hat{\assum})$. Note that
$\hat{\tau}(\hat{\assum}) = \tau_\assum
[\hat{\assum} \leftarrow \top, \assum \setminus \hat{\assum} \leftarrow \bot]$.
The only abstractions of $\bp{P}$ we consider are the ones which abstract $\tau$
and keep $\tau_B$ unchanged. That is, every abstraction $\hat{P}$ of $\bp{P}$ is
such that $\bp{P} \under_\id \hat{P}$ with $\tau(\hat{P}) = \hat{\tau}(\hat{\assum}) \land
\tau_B$ for some $\hat{\assum} \subseteq \assum$. Moreover, a subset
$\hat{\assum}$ of $\assum$  induces an abstraction of $\bp{P}$,
denoted $\bp{P}(\hat{\assum})$.


\subheading {Under-approximations} An under-approximation is induced
by a subset of assumptions $\hat{\assum} \subseteq \assum$, which
identifies the abstraction $\bp{P}(\hat{\assum})$, and a mapping
$\bvals : B \to \nat$ from $B$ to natural numbers, which bounds the
number of iterations of every loop in $\bp{P}$.  The
under-approximation, denoted $U(\hat{\assum},\bvals)$, satisfies
$U(\hat{\assum},\bvals) \sunder_\id \bp{P}(\hat{\assum})$, with
$\tau(U(\hat{\assum},\bvals)) = \hat{\tau}(\hat{\assum}) \land
\tau_B(\bvals)$ where $\tau_B(\bvals)$ is obtained from $\tau_B$ by
strengthening all transitions with $\bigand_{b \in B} b \le
\bvals(b)$.

\subheading {\textsc{Solve}}
%
We implement \solver (see Fig.~\ref{fig:code}) by transforming the
decidable under-approximation $U$, after restricting by the invariants to
$U_\invar$, to Horn-SMT~\cite{gpdr} (the input
format of $\mu Z$) and passing the result to \muz. Note that this
intentionally limits the power of \muz to solve only decidable problems.
In Section~\ref{sec:results}, we compare \algo \mbox{with~unrestricted~\muz}.

%\scnote{Discard or rewrite this para.} This transformation is a
%straightforward mapping of the individual transitions. During
%verification, $\mu Z$ computes and maintains facts which
%over-approximate reachable states at a location in at most $k$ steps,
%for $k \ge 0$. The facts at the largest $k$ denote inductive facts and
%we use this feature to add known {\em invariants} when solving a new
%under-approximation (line $5$ in Fig.~\ref{fig:code}). The facts for a
%depth $k$ are iteratively computed relative to already known facts at
%depth $\le k$. Thus, we also add the {\em lemmas} computed for a
%previous under-approximation as facts at depth $0$, acting as {\em
%  hints} to the solver. In the best case, these facts are propagated
%all the way to the largest $k$ to become lemmas of the new program. In
%other cases, they might help in a quicker propagation of other facts
%to larger depths.
%

\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{l|ll@{\makebox[3em][r]{(\rownumber)\space}}}

\multirow{6}{*}{\emph{Global}}
& \quad \multirow{2}{*}{\emph{Trans}}
& \quad $\rtag {i} {j} \implies \tau_\assum (\ell_i, \ell_j) \land \tau_B (\ell_i, \ell_j)$,
	\quad $\ell_i, \ell_j \in L$ \\

& & \quad $\ltag {i} \implies \bigor_j \rtag {j} {i}$,
	\quad $\ell_i \in L$ \\
\\
& \quad \multirow{2}{*}{\emph{Invars}}
& \quad $\left( \bigor_j \rtag{i}{j} \right) \implies \varphi$,
	\quad $\ell_i \in L$, $\varphi \in \invar (\ell_i)$ \\
& & \quad $\ltag{i} \implies \varphi'$,
	\quad $\ell_i \in L$, $\varphi \in \invar (\ell_i)$ \\

\\
\hline
\\

\multirow{9}{*}{\emph{Local}}
& \quad \multirow{2}{*}{\emph{Lemmas}}
& \quad $\bigand_{\ell_i \in L, \varphi \in \pi(\ell_i)}
		\left( \mathcal{A}_{\ell_i, \varphi} \implies
		\left( \left( \bigor_j \rtag{i}{j} \right) \implies \varphi \right) \right)$ \\
& & \quad $\neg \bigand_{\ell_i \in L, \varphi \in \pi(\ell_i)}
		\left( \mathcal{B}_{\ell_i, \varphi} \implies
		\left( \ltag{i} \implies \varphi' \right) \right)$ \\
\\
& \quad \multirow{2}{*}{\emph{Assump. Lits}}
& \quad $\mathcal{A}_{\ell, \varphi}$, \quad $\ell \in L$, $\varphi \in \pi(\ell)$ \\
& & \quad $\neg \mathcal{B}_{\ell, \varphi}$, \quad $\ell \in L$, $\varphi \in \pi(\ell)$ \\
\\
& \quad \emph{Concrete}
& \quad $\Sigma$ \\
\\
& \quad \emph{Bound Vals}
& \quad $b \le \bvals(b)$, \quad $b \in B$ \\
\end{tabular}
\caption{Constraints used in our implementation of \algo.}
\label{fig:cons}
\end{figure}


We implement the routines of \algo in Fig.~\ref{fig:code} by
maintaining a set of constraints $\mathcal{C}$ as shown in
Fig.~\ref{fig:cons}. Initially, $\mathcal{C}$ is {\em Global}.
\emph{Trans} encodes the transition relation of $\bp{P}$, using fresh
Boolean variables for transitions and locations ($\rtag{i}{j}$,
$\ltag{i}$, respectively) enforcing that a location is reachable only
via one of its (incoming) edges. Choosing an abstract or concrete
transition relation is done by adding a subset of $\assum$ as additional
constraints.  \emph{Invars} encodes currently known
invariants.  They approximate the reachable states by adding constraints for
every invariant at a location in terms of current-state variables (3)
and next-state variables (4).  The antecedent in (3) specifies that at
least one transition from $\ell_i$ has been taken implying that the
current location is $\ell_i$ and the antecedent in (4) specifies that
the next location is $\ell_i$.

$\mathcal{C}$ is modified by each routine as needed by adding and
retracting some of the \emph{Local} constraints (see
Fig.~\ref{fig:cons}) as discussed below.

For a set of \emph{assumption literals}
$\mathcal {A}$,
let \textsc{Sat}$(\mathcal{C}, \mathcal{A})$ be a function that checks whether
$\mathcal{C} \cup \mathcal{A}$
is satisfiable, and if not, returns an \emph{unsat
core} $\hat{\mathcal{A}} \subseteq \mathcal{A}$ such that $\mathcal{C} \cup
\hat{\mathcal{A}}$ is unsatisfiable. 

In the rest of the section, we assume that $\pf$ is a safety proof of
$U_\invar(\hat{\assum},\bvals)$.

\subheading {\textsc{InitU}} The initial under-approximation is
$U(\assum, \lambda b\in B \such 0)$. 

\noindent
\textbf {\textsc{ExtractInvs}} is implemented by
\textsc{ExtractInvsImpl} shown in Fig.~\ref{fig:impl_code}. It extracts
a \emph{Maximal Inductive Subset} (MIS) of the lemmas in $\pf$
w.r.t. the concrete transition relation $\tau \land \tau_B$ of
$\bp{P}$.  First, the constraints \emph{Concrete} in
Fig.~\ref{fig:cons} are added to~$\mathcal{C}$, including all of
$\assum$. Second, the constraints \emph{Lemmas} in Fig.~\ref{fig:cons}
are added to~$\mathcal{C}$, where fresh Boolean variables
$\mathcal{A}_{\ell,\varphi}$ and $\mathcal{B}_{\ell,\varphi}$ are used to mark every lemma
$\varphi$ at every location $\ell \in L$. This encodes the negation of
the inductiveness condition of a safety proof (see
Def.~\ref{def:proof}).


The MIS of $\pf$ corresponds to the \emph{maximal} subset $I \subseteq
\{\mathcal{A}_{\ell,\varphi}\}_{\ell,\varphi}$ such that $\mathcal{C} \cup I \cup \{\neg
\mathcal{B}_{\ell,\varphi} \mid \mathcal{A}_{\ell,\varphi} \not \in I\}$ is unsatisfiable.
%
$I$ is computed by \textsc{ExtractInvsImpl} in
Fig.~\ref{fig:impl_code}. Each iteration of \textsc{ExtractInvsImpl}
computes a \emph{Minimal Unsatisfiable Subset} (MUS) to identify (a minimal set
of) more non-inductive lemmas (lines~3--6). $M$, on line~4, indicates the
cumulative set of non-inductive lemmas and $X$, on line~5, indicates all the other
lemmas.  $\textsc{Mus}(\mathcal{C},T,V)$ in Fig.~\ref{fig:impl_code}
iteratively computes a minimal subset, $R$, of $V$ such that $\mathcal{C}
\cup T \cup R$ is unsatisfiable.

%by returning a \emph{minimal} subset $R$ of $V$, such that . This is
% done by incrementally adding elements of $J$ to $R$ (line $10$) whose
% negation is consistent with $\mathcal{C}$, $I$ and the current value of $R$
% (line $9$). \textbf{AG: cannot parse from here, until\ldots} In our
% case, setting an element of $J$ to {\tt false} to satisfy $\mathcal{C}$
% corresponds to making a $B_{\ell,\varphi}$ {\tt true}. This, in turn,
% corresponds to making (6) in Fig.~\ref{fig:cons} {\tt true} (assuming
% all other constraints in $\mathcal{C}$) by making $\varphi$ {\tt false} at
% the destination location $\ell$ of a transition.  Note that $R$ is
% minimal only if the necessary subset of
% $\{B_{\ell,\varphi}\}_{\ell,\varphi}$ are set to {\tt true} in a
% satisfying model. \textbf{AG: here}


\begin{figure}[t]
	\begin{subfigure}[t]{.57\textwidth}
	\begin{algorithm}[H]
	\scriptsize
	\DontPrintSemicolon

	{\sc ExtractInvsImpl}$(\mathcal{C}, \{\mathcal{A}_{\ell, \varphi}\}_{\ell,\varphi},
\{\mathcal{B}_{\ell,\varphi}\}_{\ell,\varphi})$\;
	\Begin {
\nl		$M$ := $\emptyset$, $X$ := $\{\mathcal{A}_{\ell,\varphi}\}_{\ell,\varphi}$, $Y$ :=
$\{\neg \mathcal{B}_{\ell,\varphi}\}_{\ell,\varphi}$\;
\nl		$T$ := $X$\;
		%\While {{\tt true}} {
\nl		\While {$(S := \textsc{Mus}(\mathcal{C},T,Y)) \neq \emptyset $ } {
\nl			$M$ := $M \cup S$, $Y$ := $Y \setminus M$\;
\nl			$X$ := $\{\mathcal{A}_{\ell,\varphi} ~|~ \neg
\mathcal{B}_{\ell,\varphi} \in Y\}$\;
\nl			$T$ := $X \cup M$\;
		}
\nl		\Return $X$
	}
	\end{algorithm}
	\end{subfigure}
	\begin{subfigure}[t]{.45\textwidth}
	\begin{algorithm}[H]
	\scriptsize
	\DontPrintSemicolon
    	\setcounter{AlgoLine}{7}

	{\sc Mus}$(\mathcal{C}, T, V)$\;
	\Begin {
\nl		$R$ := $\emptyset$\;
\nl		\While {{\sc Sat}$(\mathcal{C}, T \cup R)$} {
\nl			$m$ := {\sc GetModel}$(\mathcal{C}, T \cup R)$\;
\nl			$R$ := $R \cup \{v \in V ~|~ m(\neg v)\}$\;
		}
\nl		\Return $R$\;
	}
%	{\sc NextUImpl}$(B:\ubs, \mathcal{C}:\ctx)$\;
%    	\SetKwData{Global}{{\bf global}}
%	\Global {$\hat{\assum} :$ assumptions}\;
%	\Begin {
%\nl		$M$ := $\emptyset$, $\bvals : B \to \rat$\;
%\nl		\While {{\sc Sat}$(\mathcal{C}, \hat{\assum})$} {
%\nl			$m$ := {\sc Model} $(\mathcal{C})$ \;
%\nl			add $\bigor_{b \in B} (b < m(b))$ to $\mathcal{C}$\;
%\nl			add $m$ to $M$\;
%		}
%\nl		$\hat{\assum}$ := \textsc{UnsatCore}$(\mathcal{C})$\;
%\nl		$\bvals : b \in B \mapsto \min_{m \in M} m(b)$\; 
%\nl		\Return $(\bvals)$
%	}
	\end{algorithm}
	\end{subfigure}
%\vspace{-0.2in}
\caption {Our implementation of \textsc{ExtractInvs} of Fig.~\ref{fig:code}.}
\label {fig:impl_code}
%\vspace{-0.2in}
\end{figure}


\noindent
\textbf{\textsc{Abstract}} finds a $\hat{\assum}_1 \subseteq \assum$
such that $U_\invar(\hat{\assum}_1,\bvals)$ is safe with proof $\pf$. The
constraints \emph{Lemmas} in Fig.~\ref{fig:cons} are added to $\mathcal{C}$
to encode the negation of the conditions in
Definition~\ref{def:proof}. Then, the constraints in \emph{Bound Vals}
in Fig.~\ref{fig:cons} are added to $\mathcal{C}$ to encode the
under-approximation. This reduces the check for $\pf$ to be a safety
proof to that of unsatisfiability of a formula. Finally, {\sc
  Sat}$(\mathcal{C}, \assum \cup \{\mathcal{A}_{\ell,\varphi}\}_{\ell,\varphi} \cup
\{\mathcal{B}_{\ell,\varphi}\}_{\ell,\varphi})$ is invoked. As $\mathcal{C}$ is
unsatisfiable assuming $\assum$ and using all the lemmas (since $\pf$
proves $U_\invar(\hat{\assum}, \bvals)$), it returns an unsat core.
Projecting the core onto $\assum$ gives us $\hat{\assum}_1 \subseteq
\assum$ which identifies the new abstraction and, together with
$\bvals$, the corresponding new under-approximation. The minimality of
$\hat{\assum}_1$ depends on the algorithm for extracting an unsat
core, which is part of the SMT engine of Z3 in our case. In practice,
we use a \emph{Minimal Unsatisfiable Subset} (MUS) algorithm to find a
minimal $\hat{\assum}_1$. As we treat
$\{\mathcal{A}_{\ell,\varphi}\}_{\ell,\varphi}$ and
$\{\mathcal{B}_{\ell,\varphi}\}_{\ell,\varphi}$ as assumption literals, this
also corresponds to using only the necessary lemmas during
abstraction.


\subheading{\textsc{NextU}}
Given the current valuation $\bvals$ and the new abstraction $\hat{\assum}$,
this routine returns $U(\hat{\assum}, \lambda b \in B  \such \bvals(b) + 1)$.

%We create a new
%incremental context $\mathcal{C}_A$, on top of $\mathcal{C}_L$, and assert all
%the $a_{\ell,\varphi}$s and $b_{\ell,\varphi}$s selecting all the
%lemmas in $\pf$. Note again that we do not assert $\bvals$ into our
%context as we want to {\em obtain} a new $\bvals$ and choose a new
%abstraction such that $\pf$ still holds for the resulting
%under-approximation.  We obtain both using a single algorithm {\sc
%  NextUImpl}$(B,\mathcal{C}_A)$, shown in Fig.~\ref{fig:impl_code} which
%starts with checking {\sc Sat}$(\mathcal{C}_A, \hat{\assum})$ on line
%$10$. If it returns {\tt false}, as we did not impose any constraints
%on the bound variables, $\pf$ is already a proof of $\bp{P}$. This
%corresponds to an undefined $\bvals$ on line $15$. Otherwise, we add a
%constraint to look for smaller bounds than those reported by the SMT
%solver, on line $12$. This is guaranteed to terminate as the
%constraints reduce the possible values of some $b \in B$ in each
%iteration and this cannot happen forever as the current $\bvals$ is a
%lower bound. When the SMT check returns {\tt false}, we obtain the new
%$\bvals$ as the least values reported by the SMT solver so far (line
%$15$) and also obtain the new abstraction, $\hat{\assum}$, from the
%unsat core (line $14$).

\subheading {\textsc{Refine} and \textsc{IsFeasible}} Let
$U_\invar(\hat{\assum},\bvals)$ be unsafe with a counterexample $\cex$.  We
create a new set of constraints $\mathcal{C}_\cex$ corresponding to the
unrolling of $\tau_\assum \land \tau_B$ along the control path of
$\cex$ and check {\sc Sat}$(\mathcal{C}_\cex, \assum)$.  If the path is
feasible in $\bp{P}$, we find a counterexample to safety in
$\bp{P}$. Otherwise, we obtain an unsat core $\hat{\assum}_1 \subseteq \assum$ and
refine the abstraction to $\hat{\assum} \cup \hat{\assum}_1$. The
under-approximation is refined accordingly with the same $\bvals$.

We conclude the section with a discussion of the implementation
choices.  \textsc{NextU} is implemented by incrementing all bounding
variables uniformly. An alternative is to increment the bounds only for the loops
whose invariants are not inductive (\eg~\cite{ufo,impact}).
However, we leave the exploration of such
strategies for future. Our use of \muz is sub-optimal since each
call to \solver requires constructing a new Horn-SMT problem. This
incurs an unnecessary pre-processing overhead that can be eliminated
by a tighter integration with \muz. For \textsc{Abstract} and
\textsc{ExtractInvs}, we use a single SMT-context with a single copy
of the transition relation of the program (without unrolling it). The
context is preserved across iterations of \algo. Constraints specific
to an iteration are added and retracted using the incremental solving
API of Z3. This is vital for performance. For \textsc{Refine} and
\textsc{IsFeasible}, we unroll the transition relation of the program
along the control path of the counterexample trace returned by \muz. We experimented with
an alternative implementation that instead validates each individual
step of the counterexample using the same global context as
\textsc{Abstract}. While this made each refinement step faster, it
increased the number of refinements, becoming inefficient overall.





%   In summary,


% discuss: 

%   1. our choice of bounds. other options that we have not
%      explored. namely nextU. Can pick bounds non-uniformly.

%   2. for abstraction and proof feasibility: use single context for the
%   transition relation of the program. no unrolling.

%   3. for counterexamples, unroll the transition relation along a
%   pass. We have experimented with refining without unrolling as well,
%   but this was not effective.


% In summary, we described our implementation of \algo by means of extra
% constraints on the transitions to obtain decidable
% under-approximations, treating all variables in $C$ uniformly and
% incrementing each bound variable in $B$ by 1 for a new
% under-approximation. 

% It would be interesting to explore other alternatives.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> paper.tex <==
\input{main}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

